Fog Device-as-a-Service (FDaaS): A Framework for Service Deployment in Public Fog Environments

Meeting the requirements of future services with time sensitivity and handling sudden load spikes of the services in Fog computing environments are challenging tasks due to the lack of publicly available Fog nodes and their characteristics. Researchers have assumed that the traditional autoscaling techniques, with lightweight virtualisation technology (containers), can be used to provide autoscaling features in Fog computing environments, few researchers have built the platform by exploiting the default autoscaling techniques of the containerisation orchestration tools or systems. However, the adoption of these techniques alone, in a publicly available Fog infrastructure, does not guarantee Quality of Service (QoS) due to the heterogeneity of Fog devices and their characteristics, such as frequent resource changes and high mobility. To tackle this challenge, in this work we developed a Fog as a Service (FaaS) framework that can create, configure and manage the containers which are running on the Fog devices to deploy services. This work presents the key techniques and algorithms which are responsible for handling sudden load spikes of the services to meet the QoS of the application. This work provides an evaluation by comparing it with existing techniques under real scenarios. The experiment results show that our proposed approach maximises the satisfied service requests by an average of 1.9 times in different scenarios.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Result/Finding_2_graphs <==

FInding 2 bar graphs

set xtics rotate by -45



reset
fontsize = 12
set term postscript enhanced eps fontsize
set output "Ravg.eps"
set key box left top vertical
set style fill solid 2.00 border 0
set style histogram errorbars gap 2 lw 1
set style data histogram
set grid ytics
set xlabel "Rates"
set ylabel "Average number of failures"
set yrange [0:*]
set datafile separator ","
plot 'c.dat' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2

__________________________________________________________________________________

reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '5fail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '5fail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '5res.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '5res' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '10fail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '10fail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '10res.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '10res' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2







reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '15fail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '15fail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '15res.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '15res' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '20fail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '20fail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '20res.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '20res' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2



reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '25fail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '25fail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output '25res.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Number of devices" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot '25res' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2




reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Ravgfail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'Ravgfail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Ravgdel.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'Ravgdel' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2




reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Navgfail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'Navgfail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Navgdel.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'Navgdel' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Ravgfail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'Ravgfail' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Ravgdel.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'Ravgdel' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2




reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'failmul.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'failmul' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'resmul.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'resmul' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2



reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'nfailmul.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average number of failures" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'nfailmul' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2





reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'nresmul.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 2
set style histogram errorbars gap 2 lw 2
set style data histogram
set grid ytics
set xlabel "Rates" offset 0,0.5,0
set ylabel "Average processing time (sec)" offset 2,0,0
set yrange [0:*]
set datafile separator "\t"
plot 'nresmul' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2













_______________________________________________________________________________________________
reset
set terminal postscript eps enhanced font "Helvetica,24"
set output 'Ravgfail.eps'
set key samplen 2.1 spacing 1 font ",24"
set key width -3
set key box outside center top horizontal
set style fill solid 1.00 border 0
set style histogram errorbars gap 2 lw 1
set style data histogram
set grid ytics
set xlabel "Rates"
set ylabel "Average processing time (sec)"
set yrange [0:*]
set datafile separator "\t"
plot 'Ravgfail.dat' using 2:3:xtic(1) ti "NLBF"lc rgb 'black' lw 1 fillstyle pattern 4, \
'' using 4:5 ti "Best-Fit" lc rgb 'black' lt 1 lw 1 fillstyle pattern 2







set key at graph 0.1, 0.9



